Measurements of Beam Backgrounds in SuperKEKB Phase 2

The high design luminosity of the SuperKEKB electron-positron collider will result in challenging levels of beam-induced backgro\ unds in the interaction region. Understanding and mitigating these backgrounds is critical to the success of the Belle~II experi\ ment. We report on the first background measurements performed after roll-in of the Belle II detector, a period known as SuperKE\ KB Phase 2, utilizing both the BEAST II system of dedicated background detectors and the Belle II detector itself. We also repor\ t on first revisions to the background simulation made in response to our findings. Backgrounds measured include contributions f\ rom synchrotron radiation, beam-gas, Touschek, and injection backgrounds. At the end of Phase 2, single-beam backgrounds origina\ ting from the 4 GeV positron Low Energy Ring (LER) agree reasonably well with simulation, while backgrounds from the 7 GeV elect\ ron High Energy Ring (HER) are approximately one order of magnitude higher than simulation. We extrapolate these backgrounds for\ ward and conclude it is safe to install the Belle II vertex detector.

==> 07_Injection_BG_Study_and_Mitigation/Ch_7_Injection_BG_Study_and_Mitigation.tex <==
% !TeX root = ../beast_phase2.tex


\section{Injection BG Study and Mitigation}
\label{sec:injection_study}
\index{Injection BG Study and Mitigation}


\subsection{Study Description}
On July 13th, 2018, a dedicated injection study using the high energy ring was carried out. Various parameter such as injection phase and beam energy of the injected bunches or septum angle and kicker height at the linear accelerator collider interface and more can be varied in order to change the particle loss induced by particle injections. A fixed injection pattern filling the high energy ring to a maximum of $200\,\mathrm{mA}$ in two steps at a fixed rate of $12\,\mathrm{Hz}$ with the lowest possible injection bunch current enables comparability among the parameter modifications. In the first step, the high energy ring is filled from $0\,\mathrm{mA}$ to $100\,\mathrm{mA}$ beam current. Injections after a current drop of $1\,\%$ keep the beam current stable over a period of around $5\,\mathrm{min}$ before the collider is filled up to $200\,\mathrm{mV}$. For the time of the study, the low energy ring was kept at zero beam current.
Reference data taken before the study and with default parameters ensure comparability.
\par
Reference data with default injection parameters was taken prior to the study. These runs are referred to as \textit{ref-inj}. Data taken during injections is indicated with \textit{inj} and non injection data is referred to as \textit{non-inj}.


\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.45\textwidth]{time_in_turn_herInj_fnorm=1000}
  \caption{Calculated $Z_{eff}$ values for the final month of Phase~2 running.}
  \label{fig:time_in_turn_herInj}
\end{figure}


\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.45\textwidth]{time_in_turn_nonInj_fnorm=1000}
  \caption{Calculated $Z_{eff}$ values for the final month of Phase~2 running.}
  \label{fig:time_in_turn_nonInj}
\end{figure}


==> 08_Synchrotron_Radiation/Ch_8_Synchrotron_Radiation.tex <==
\subsection{Synchrotron Radiation}
\label{sec:synchrotron}
\index{Synchrotron Radiation}


